AutoWebGLM: A Large Language Model-based Web Navigating Agent

Large language models (LLMs) have fueled many intelligent web agents, but most existing ones perform far from satisfying in real-world web navigation tasks due to three factors: (1) the complexity of HTML text data (2) versatility of actions on webpages, and (3) task difficulty due to the open-domain nature of the web. In light of these challenges, we develop the open AutoWebGLM based on ChatGLM3-6B. AutoWebGLM can serve as a powerful automated web navigation agent that outperform GPT-4. Inspired by human browsing patterns, we first design an HTML simplification algorithm to represent webpages with vital information preserved succinctly. We then employ a hybrid human-AI method to build web browsing data for curriculum training. Finally, we bootstrap the model by reinforcement learning and rejection sampling to further facilitate webpage comprehension, browser operations, and efficient task decomposition by itself. For comprehensive evaluation, we establish a bilingual benchmark -- AutoWebBench -- for real-world web navigation tasks. We evaluate AutoWebGLM across diverse web navigation benchmarks, demonstrating its potential to tackle challenging tasks in real environments. Related code, model, and data are released at \url{https://github.com/THUDM/AutoWebGLM}.

==> tables/annotation_document.tex <==
\begin{table*}[htbp]
\caption{Annotation Documentation.}
	\renewcommand\arraystretch{1.2}
\label{tab:annotation_document}
\resizebox{\textwidth}{!}{

\begin{tabular}{rp{0.82\textwidth}}
\toprule
Annotation Target & We collected several websites and generated 50 unique tasks for each. For each website, annotators must perform operations according to the task descriptions to complete the requirements. \\
\midrule
Installation of Plugin & We recommend using Google Chrome for annotation. \\                                                                        
1 & Download the plugin code zip package. \\
2 & Download the annotation data and place the folder in the directory where your plugin code is located.   \\
3 & Start Chrome, go to More > More Tools > Extensions, enable Developer mode and load the unpacked extension by selecting the unzipped plugin code directory. \\
\midrule
Plugin Introduction & To learn how to use the plugin in detail, please refer to the \href{https://cloud.tsinghua.edu.cn/d/675b301ef51c4bc3aa0d/}{introduction video}. The plugin has three main functions: Start/Pause Recording, End Recording, and Record Archive. \\
& Navigation between websites and tasks is made easier with the use of '«' and '»' for previous and next websites, and '<' and '>' for previous and next tasks. The plugin also provides input fields for direct navigation. \\
\cmidrule{2-2}
1& Click the trash bin icon to reset the environment.\\
2& When encountering login or robot authentication, add an authorization record by clicking the plus (+) icon one step before the corresponding operation.\\
3& If the task requires an answer, click the plus (+) icon in the appropriate place to insert and edit the answer.\\
4& If there is no response when you type content into an input field, click the plus sign and go to the appropriate location to insert and edit the input content (note that the input field is the last object to be clicked, so make sure the last click was on an input field).\\
5& By default, the navigation record is marked as automatic. For manual navigation, such as typing a URL or going to the previous or next page, click the word "Navigation" in this record to change it to a manual navigation record.\\
6& Navigation operations are not recorded until the page is fully loaded. Wait for the navigation record to appear before you continue.\\
7& If you need an element on the page to hover, you can click on that element and change the "click" event to a "mouseover" record.\\
\midrule  
Annotation Process & Here is a checklist for your reference.\\
1 & Enter the assigned website number in the designated input box and navigate to the corresponding website.\\
2 & First, verify if the auto-generated website description aligns with the website's functionality. The description need not be detailed, but it should be generally correct. If it matches, proceed with annotation; otherwise, skip the website.\\
3 & Task descriptions are evaluated to determine their feasibility based on criteria such as the precision of the description, whether the task is typical of the average user of the site, and its overall feasibility. Tasks that do not involve complex login or registration operations and those that do not have too many subjective conditions are preferred. If the task has minor issues, such as an unachievable condition or involving subjective conditions, you may modify it directly in the task editing box.\\
4 & Start executing operations according to the task description, paying attention to whether there are missing or redundant operations, and handle login or robot verification as specified.
After completing the task, click "End" and then "Record Archive" to save.\\
5 & Once annotation is complete, please upload the contents of the tasks directory.\\
\midrule      
Additional Annotation & Design ten tasks for each website, with each task containing at least 15 effective steps. An operation is considered effective only if it is a click, mouseover, or input change that contributes to achieving the goal. Remove any erroneous operations from the record.\\
\cmidrule{2-2}
1 & Enter the assigned website number in the website input box and navigate to that website.\\
2 & Briefly browse the website to determine possible tasks.\\
3 & Choose a task number. The task box will not contain any data at this point.\\
4 & Start recording operations.\\
5 & After completing the operations, fill in the completed task in the task box.\\
6 & Save the result. \\
\bottomrule
\end{tabular}

}

\end{table*}

==> tables/combine_table.tex <==

\begin{table*}[t]
\caption{Benchmark Results for Various Models}
\vspace{-4mm}
\label{tab:benchmark_results}
\small
\renewcommand\tabcolsep{3pt}
\renewcommand\arraystretch{1}
\begin{tabular}{lccccccccccc}
\toprule
\multirow{5}{*}{Model} & \multirow{5}{*}{Parameter} & \multicolumn{4}{c}{AutoWebBench} & \multicolumn{4}{c}{Mind2Web} & \multicolumn{2}{c}{Others} \\
\cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(lr){11-12}
 & & \multicolumn{2}{c}{English} & \multicolumn{2}{c}{Chinese} & \multirow{3}{*}{\makecell{Cross-\\Task}} & \multirow{3}{*}{\makecell{Cross-\\Website}} & \multirow{3}{*}{\makecell{Cross-\\Domain}} & \multirow{3}{*}{Overall} & \multirow{3}{*}{MiniWoB++} & \multirow{3}{*}{WebArena} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
 & & \makecell{Cross-Task} & \makecell{Cross-Website} & \makecell{Cross-Task} & \makecell{Cross-Website} & & & & & & \\


\midrule
ChatGPT & 175B & 12.10 & 6.35 & 13.50 & 10.80 & 17.40 & 16.20 & 18.60 & 17.40 & 13.39 & 6.16 \\
GPT-4 & N/A & 38.60 & 39.70 & 36.70 & 36.30 & 36.20 & 30.10 & 26.40 & 30.90 & 32.14 & 14.41 \\
Flan-T5-XL & 3B & - & - & - & - & 52.00 & 38.90 & 39.60 & 43.50 & - & - \\
HTML-T5-XL & 540B+3B & - & - & - & - & 71.50 & 62.20 & 67.10 & 66.93 & 85.60 & - \\
CC-Net & N/A & - & - & - & - & - & - & - & - & 32.00 & - \\
WebN-T5-XL & 3B & - & - & - & - & - & - & - & - & 48.40 & - \\
Llama2 (finetuned) & 7B & - & - & - & - & - & - & - & - & - & - \\
Claude & N/A & - & - & - & - & - & - & - & - & - & - \\
\midrule
\model & & 64.81 & 58.62 & 65.36 & 61.82 & 66.35 & 56.4 & 55.8 & 59.52 & 89.30 & 18.17 \\
\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table*}

==> tables/rm_acc.tex <==


\begin{table}[htbp]
\caption{Reward Model Result.}
\label{tab:rm_acc}
\centering
\vspace{-3mm}
\renewcommand\tabcolsep{5pt}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{@{}lccccc@{}}
\toprule
 & \multicolumn{2}{c}{PRM Accuracy} & \multicolumn{2}{c}{ORM Accuracy} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
Model & \benchmark & Mind2Web & MiniWob++ & WebArena \\
\midrule
\chatgpt & 54.6 & 45.6 & - & - \\
\gptfour & 56.3 & 47.8 & - & - \\
\model & 64.8 & 68.7 & - & - \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}

==> tables/webarena_result.tex <==
\begin{table}[ht]
\caption{WebArena}
\label{tab:webarena}
\centering
\vspace{-2mm}
\renewcommand\tabcolsep{5pt}
\begin{tabular}{@{}ccccc@{}}
\toprule
Model & SR (avg.) \\ \midrule
AutoGLM & 32.28 \\
GPT-4 & 39.15 \\
GPT-3.5-Turbo & 36.50 \\
CC-Net & 32.00 \\
WebN-T5-XL & 48.4 \\
WebAgent & 36.50 \\ 
Lemur & 5.30 \\ \bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}
